X-ray observations of SU UMa throughout six outbursts

We present RXTE observations covering six normal outbursts of the dwarf nova SU UMa, the prototype of its class. The outbursts showed consistent X-ray behaviour with the X-ray count rate dropping suddenly by a factor of our, and with evidence for a half day delay between the optical rise and the X-ray suppression. In contrast to SS Cyg, an X-ray flux increase at the beginning of outburst was not observed, although it is expected from boundary layer models. The X-ray flux was high and decreasing during quiescence, in conflict with the disc instability model. The X-ray spectrum of SU UMa was softer in outburst than during quiescence, and it was consistent with constant reflection.

==> table_suuma_obs.tex <==

%%
%% table with the basic information about this observation 
%% of SU UMa.
%% data includes:
%%	Proposal ID
%%	Year
%%	Start - End Date
%%	Number of Observations
%%	Total Exposure time
%%	Gain Epoch
%%


\begin{tabular*}{\textwidth}{c@{\extracolsep{\fill}}cccc}


\hline \hline


Year &
Start - End &
Number of &
Total &
Gain \\

&Date &Observations &Exposure (ks) & Epoch\\


\hline

2001 &March 25 - June 21 &193 &336 &5 \\

\hline

\end{tabular*}




